Viscot-steer: Disentangling and Transferring Visual Chain-of-Thought via Activation Steering

Visual chain-of-thought (visual-CoT), also known as "thinking with images", equips LVLMs with the ability to locate and use key visual evidence for reasoning. However, acquiring such visual-CoT capabilities requires costly post-training and tightly couples them to a specific backbone, making transfer to other LVLMs difficult. Existing cross-model transfer methods typically treat visual-CoT as a monolithic capability, using a unified representation that ignores the functional distinction between grounding and reasoning and introduces stage-irrelevant interventions. To address this problem, we propose Viscot-steer, a training-free activation steering framework for transferring visual-CoT capabilities across heterogeneous LVLMs. Specifically, Viscot-steer first disentangles visual-CoT into grounding and reasoning vectors and extracts them from the source-model layers associated with the corresponding capabilities. It then aligns the vectors with the activation space of the target model and steers the grounding and reasoning layers during bounding-box prediction and reasoning-trace generation, respectively. Across benchmarks covering high-resolution visual understanding, general visual perception and reasoning, and mathematical visual reasoning, Viscot-steer transfers capabilities from different visual-CoT models to architecturally diverse LVLMs and outperforms the strongest capability-transfer baseline by an average of 1.86 percentage points on the primary evaluation metrics.

==> arxiv-style.tex <==
% Minimal arXiv additions; retain the original ICLR title/abstract layout.

% All theme colors are defined centrally in _macros.tex.
\newcommand{\projectpageurl}{https://nn-wang.github.io/viscot-steer}

% Draw a font-independent envelope marker for corresponding authors.
\RequirePackage{tikz}
\newcommand{\correspondingauthor}{%
  \tikz[baseline=-0.15ex,x=1em,y=1em]{%
    \draw[line width=0.3pt,line join=round]
      (0,0) rectangle (0.85,0.55);
    \draw[line width=0.3pt,line join=round]
      (0,0.55) -- (0.425,0.22) -- (0.85,0.55);
  }%
}

% Add two rows inside the original abstract's quote environment.
% Do not override \@maketitle, the abstract environment, or ICLR spacing.
\newcommand{\papercontactinfo}{%
  \par\vspace{0.5em}%
  {\raggedright\small\noindent
    \textbf{Project page:}\enspace
    \href{\projectpageurl}{%
      \textcolor{arxivaccent}{\texttt{nn-wang.github.io/viscot-steer}}}%
    \par\vspace{0.2em}%
    \noindent\textbf{Contact:}\enspace
    \textcolor{arxivaccent}{\texttt{\{nn.wang, beier.zhu, xyang21\}@ustc.edu.cn}}%
    \par
  }%
}
\AddToHook{env/abstract/end}{\papercontactinfo}

% Human-readable PDF metadata for the non-anonymous manuscript.
\hypersetup{%
  pdftitle={Viscot-steer: Disentangling and Transferring Visual Chain-of-Thought via Activation Steering},
  pdfauthor={Ningning Wang, Beier Zhu, Xingyu Zhu, Kaiyun Yang, Xun Yang}
}

